Multi-Agent Coverage in Urban Environments

We study multi-agent coverage algorithms for autonomous monitoring and patrol in urban environments. We consider scenarios in which a team of flying agents uses downward facing cameras (or similar sensors) to observe the environment outside of buildings at street-level. Buildings are considered obstacles that impede movement, and cameras are assumed to be ineffective above a maximum altitude. We study multi-agent urban coverage problems related to this scenario, including: (1) static multi-agent urban coverage, in which agents are expected to observe the environment from static locations, and (2) dynamic multi-agent urban coverage where agents move continuously through the environment. We experimentally evaluate six different multi-agent coverage methods, including: three types of ergodic coverage (that avoid buildings in different ways), lawn-mower sweep, voronoi region based control, and a naive grid method. We evaluate all algorithms with respect to four performance metrics (percent coverage, revist count, revist time, and the integral of area viewed over time), across four types of urban environments [low density, high density] x [short buildings, tall buildings], and for team sizes ranging from 2 to 25 agents. We believe this is the first extensive comparison of these methods in an urban setting. Our results highlight how the relative performance of static and dynamic methods changes based on the ratio of team size to search area, as well the relative effects that different characteristics of urban environments (tall, short, dense, sparse, mixed) have on each algorithm.

==> delete_this.tex <==
\section{Ergodic}
\subsection{Overview}
Ergodic theory is a statistical study of the time average of the dynamical system which has believed to be explored all possible states 

\subsection{Multi-agent Coverage Problem}
Coverage problem for ergodic coverage is to find $B$ such that $\spacespace{search} \backslash \spacespace{swept} = \emptyset$, where definition of $\spacespace{swept}$ is given by:
\begin{equation}\label{Eqn.3-5}
    \spacespace{swept} = \{ X \mid X \in \bigcup_{\hat{x} \in B} \spacecone{\hat{x}} \}
\end{equation}
\noindent
and where $\spacespace{search} \subseteq \spacespace{swept}$ and $ B = \bigcup_{j =1}^{N} \{B_j\}$.
where,
\begin{equation}\label{Eqn.5}
    B_j(t) = \sum_{R} \Lambda_{k} S_{k} \nabla f_k(x_j(t))
\end{equation}

$S_k(t) := C_k(t) - M_k(t)$ \\
$$\nabla f_k(x_j(t)) = \frac{1}{h_k} \left[ 
\begin{array}{c}
    -k_1 \sin(k_1x_1)\cos(k_2x_2) \\
    -k_2 \cos(k_1x_1)\sin(k_2x_2) 
\end{array}
\right]$$ \\
$C_k(t) := Nt\fourcoeffc$ \\
$M_k(t) := Nt\fourcoeffu$ \\
$f_k(x) = \frac{1}{h_k} \cos(k_1x_1)\cos(k_2x_2)$ \\
$k_1 = \frac{K_1\pi}{L_1}$, $k_2 = \frac{K_2\pi}{L_2}$ \\
$$\fourcoeffc = \frac{1}{Nt} \sum_{j=1}^{N} \int_{0}^{t} f_k(x_j(\tau))d\tau$$ \\
$\fourcoeffu = \langle \mu, f_k \rangle$, where $\langle \cdot,\cdot\rangle$ is an inner product.\\
$$h_k = \left( \int_{0}^{L_1} \int_{0}^{L_2} \cos^2(k_1x_1) \cos^2(k_2x_2) \right)^{1/2}$$


==> delete_this_2.tex <==
\section{Lawn mower}
\subsection{Overview}
As mentioned earlier, this method is also known as boustrophedon Coverage which is widely popular due to it's simplicity and guaranteed 100\% coverage. Urban environment has its own challenges compare to conventional two dimensional approaches. Main problem was the coverage of occluded areas created by the densely constructed buildings and was mitigated by going over the building for their coverage.

\subsection{Multi-agent Coverage Problem}
Coverage problem for Lawn Mower is to find $\pathset$ such that $\spacespace{search} \backslash \spacespace{swept} = \emptyset$, where definition of $\spacespace{swept}$ is given by:
\begin{equation}\label{Eqn.3-4}
    \spacespace{swept} = \{ X \mid X \in \bigcup_{\hat{x} \in \varrho} \spacecone{\hat{x}} \}
\end{equation}
\noindent
and where $\spacespace{search} \subseteq \spacespace{swept}$ and $ \pathset = \bigcup_{i =1}^{n} \{\rho_i\}$.
